Net2: A Graph Attention Network Method Customized for Pre-Placement Net Length Estimation

Net length is a key proxy metric for optimizing timing and power across various stages of a standard digital design flow. However, the bulk of net length information is not available until cell placement, and hence it is a significant challenge to explicitly consider net length optimization in design stages prior to placement, such as logic synthesis. This work addresses this challenge by proposing a graph attention network method with customization, called Net2, to estimate individual net length before cell placement. Its accuracy-oriented version Net2a achieves about 15% better accuracy than several previous works in identifying both long nets and long critical paths. Its fast version Net2f is more than 1000 times faster than placement while still outperforms previous works and other neural network techniques in terms of various accuracy metrics.

==> _txt/del_background.tex <==
\section{Preliminary // move to intro/method}

\subsection{Graph Neural Network}
\label{GNN}

In recent years, deep learning has achieved astonishing impact in many filed, from image classification to natural language understanding, where tasks are represented in Euclidean space. However, there are a wide range of applications where data are represented in the form of graphs. Conducting learning algorithms on graphs is significantly more challenging and has been intensively studied in deep learning community. Here we refer all neural network-based methods on graph as graph neural networks (GNN). The most widely-used GNN methods include GCN \cite{kipf2016semi}, GraphSage \cite{hamilton2017inductive}, and Graph Attention Network (GAT) \cite{velivckovic2017graph}. All these three methods perform an operation named \emph{spatial-based convolution}, which convolves the central node's representation with its neighbors' representations to derive an updated representation for the central node. Such operation essentially propagates node information along edges.

For a node $k$ with node features $O_k$, denote its embedding at the $t$ layer as $h_k^{(t)}$. Its initial embedding is the node features $h_k^{(1)} = O_k$. Dentoe the collection of its neighbors $b$ as $\mathcal{N}(k)$, where $b \in \mathcal{N}(k)$. The degree of this node means the number of its neighbors: $deg(k) = len(\mathcal{N}(k))$. For all GNN methods mentioned above, in each layer $t$, they calculates the updated embedding $h_k^{(t)}$ based on the previous embedding of the node itself $h_k^{(t-1)}$ and its neighbors $h_b^{(t-1)} | b\in \mathcal{N}(k)$:

\begin{gather*}
h_k^{(t)} = \mathcal{F}_{GCN/Sage/GAT}^{(t)} (h_k^{(t-1)}, h_b^{(t-1)} ), \forall b \in \mathcal{N}(k)
\end{gather*}


We show one layer of each aforementioned GNN below. The two-dimensional learnable weight at layer $t-1$ is $W^{(t-1)}$. It can also be viewed as the weight of one-layer neural network. In GAT, there is an extra one-dimensional weight shared in all layers, denoted as $\theta$. The expression $[ || ]$ means concat two vectors into one longer vector. Functions $\sigma$ and $g$ are sigmoid activation function and Leaky ReLu activation function, respectively.

On GCN (with self-loops), $\mathcal{F}_{GCN}^{(t)}$ is:
\begin{gather*}
  h_k^{(t)} = \sigma (\sum_{b\in {\mathcal{N}(k) \cup k}} c_{kb} h_b^{(t-1)} W^{(t-1)}) \\
  \text{where   } c_{kb} = \frac{1}{\sqrt{deg(k) + 1} \sqrt{deg(b) + 1}}
\end{gather*}

On GraphSage (with mean aggregator), $\mathcal{F}_{Sage}^{(t)}$ is:
\begin{gather*}
  h_k^{(t)} = \sigma ( W^{(t-1)} [h_k^{(t-1)} || \frac{1}{deg(k)} \sum_{b\in {\mathcal{N}(k)}}  h_b^{(t-1)}]) 
\end{gather*}

On GAT, $\mathcal{F}_{GAT}^{(t)}$ is:
\begin{gather*}
  h_k^{(t)} = \sigma (\sum_{b\in {\mathcal{N}(k) \cup k}} c_{kb} h_b^{(t-1)} W^{(t-1)}) \\
  \text{where   } c_{kb} = \sigma (g (\theta[ h_b^{(t-1)} W^{(t-1)} || h_k^{(t-1)} W^{(t-1)} ]))
\end{gather*}



Notice that there are many other variations and expressions of these methods. Here we choose the variation used in our experiment and present them with a rather consistent expression.


\subsection{GNN in EDA}

For machine learning applications in EDA, data is usually in Euclidean space after placement finishes, which inspired many convolutional neural network (CNN) or generative adversarial network (GAN)-based methods \cite{xie2018routenet}\cite{yu2019painting}\cite{fang2018machine}. But before placement, graph becomes a core data format and spatial information is no longer directly available. Until recent years, we start to witness some early EDA works based on GNN methods. For example, \cite{ma2019high} predict observation point candidates in a netlist. It's algorithm is almost the same as GraphSage \cite{hamilton2017inductive}. Graph-CNN \cite{zhang2019circuit} predicts the electromagnetic propertyies of distributed circuits, with algorithms similar to GAT \cite{velivckovic2017graph}. This work is verified on an extremely simple graph with less than ten nodes.



